COVID-19 Activity Risk Calculator as a Gamified Public Health Intervention Tool

The Coronavirus disease 2019 (COVID-19) pandemic, caused by the virus severe acute respiratory syndrome coronavirus 2 (SARS-CoV-2), has impacted over 200 countries leading to hospitalizations and deaths of millions of people. Public health interventions, such as risk estimators, can reduce the spread of pandemics and epidemics through influencing behavior, which impacts risk of exposure and infection. Current publicly available COVID-19 risk estimation tools have had variable effectiveness during the pandemic due to their dependency on rapidly evolving factors such as community transmission levels and variants. There has also been confusion surrounding certain personal protective strategies such as risk reduction by mask-wearing and vaccination. In order to create a simple easy-to-use tool for estimating different individual risks associated with carrying out daily-life activity, we developed COVID-19 Activity Risk Calculator (CovARC). CovARC is a gamified public health intervention as users can "play with" how different risks associated with COVID-19 can change depending on several different factors when carrying out routine daily activities. Empowering the public to make informed, data-driven decisions about safely engaging in activities may help to reduce COVID-19 levels in the community. In this study, we demonstrate a streamlined, scalable and accurate COVID-19 risk calculation system. Our study also demonstrates the quantitative impact of vaccination and mask-wearing during periods of high case counts. Validation of this impact could inform and support policy decisions regarding case thresholds for mask mandates, and other public health interventions.

==> hosp_death_old.tex <==
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}\\ \hline\end{tabular}                                              
                                                                                                                                                                                                   & \textit{\textbf{Hospitalization					Rate					(\%)}}          & \textit{\textbf{Death					Rate					(\%)}}                        &   \\ \hline
\textit{\textbf{By					Age					Group					a					[1],					[2]}}                                                                                                                                                                                                                              &                                                              &                                                                  &   \\ \hline
0-17
					years                                                                                                                                                                                                                                                                            & 0.8\%                                                        & 0.0015\%                                                         &   \\ \hline
18-49
					years                                                                                                                                                                                                                                                                           & 2.5\%                                                        & 0.07\%                                                           &   \\ \hline
50-64
					years                                                                                                                                                                                                                                                                           & 7.9\%                                                        & 0.7\%                                                            &   \\ \hline
65+
					years                                                                                                                                                                                                                                                                             & 23\%                                                         & 6\%                                                              &   \\ \hline
All
					ages                                                                                                                                                                                                                                                                              & 5\%                                                          & 0.75\%                                                           &   \\ \hline
\textit{\textbf{By					SARS-CoV-2					Variant-					Fold					Higher					Risk					Compared					to					Original					Variants}}                                                                                                                                                                &                                                              &                                                                  &   \\ \hline
Alpha
					(B.1.1.7
					B.1.1.7
					with
					E484K)                                                                                                                                                                                                                                     & 1.5					(1.5–1.6)					c					[3]                              & 1.6					(1.4–1.7)					[3]                                        &   \\ \hline
Beta
					(B.1.351)                                                                                                                                                                                                                                                                        & Under
					Investigation                                     & Possibly					increased					[4,					7]                            &   \\ \hline
Gamma
					(P.1)                                                                                                                                                                                                                                                                           & Possibly					Increased					[4]                               & 1.5					(1.2–1.9)					e,					f					[8,					9]                    &   \\ \hline
Delta
					(B.1.617.2)                                                                                                                                                                                                                                                                     & 2.3					(1.9–3.0)					d,					e					[5,					6]                & 2.4					(1.5–3.3)					[6]                                        &   \\ \hline
\textit{\textbf{By					Gender					-					Fold					Higher					Risk					g					[10]					[12]}}                                                                                                                                                                                                 &                                                              &                                                                  &   \\ \hline
Male                                                                                                                                                                                                                                                                                       & -                                                            & 1.5-2.3                                                          &   \\ \hline
Female                                                                                                                                                                                                                                                                                     & -                                                            & 1                                                                &   \\ \hline
\textit{\textbf{By					Any					Chronic					Health					Condition					-					Fold					Higher					Risk					[11][12]}}                                                                                                                                                                          &                                                              &                                                                  &   \\ \hline
\begin{tabular}[c]{@{}l@{}}Diabetes,					Heart					Disease,					Cancer,					Lung					disease,					High					Blood					Pressure,					\\ \hline					Immunocompromised,					Asthma,					Kidney					Disease,					Obesity,					Sickle					Cell					Anemia,					HIV,					Liver					Disease.\end{tabular} & \begin{tabular}\scalebox{0.1}[c]{@{}l@{}}\\ \hline															2.5\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ \hline															1.2-6.9\end{tabular} &  
\end{tabular}
\end{table}

==> old_comparison_table.tex <==
% \begin{table}
% \centering
% \scalebox{0.55}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l} 
% \hline

% \multirow{\textbf{~ ~ ~ RISK CALCULATOR }}                                                              & \multicolumn{12}{l|}{~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~  \textbf{CRITERIA}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ 
% \cline{2-14}
%                                                                                                         & User-friendly UI & \begin{tabular}[c]{@{}l@{}}Vaccination\end{tabular} & \begin{tabular}[c]{@{}l@{}}Health\\conditions\end{tabular} & \begin{tabular}[c]{@{}l@{}}Many\\locations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Masks\\and mask\\ types\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of\\people\end{tabular} & \begin{tabular}[c]{@{}l@{}}If\\indoor or\\outdoor~\end{tabular} &  \begin{tabular}[c]{@{}l@{}}Specific\\activities\end{tabular} & \begin{tabular}[c]{@{}l@{}}Calc.\\risk of\\infection\end{tabular} & \begin{tabular}[c]{@{}l@{}}Calc.\\risk of\\hospitalization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Calc.\\risk of\\death\end{tabular} & Shows working  \\ 
% \hline
% Our model                                                                                               & ~ ~ ~ ~ ~ ~ ~ X                & ~ ~ ~ ~X                                                       & ~ ~ ~ ~ X                                                            & ~ ~ ~ ~X                                                          & ~ ~ ~ ~X                                                                & ~ ~ ~ ~ X                                                           & ~ ~ ~ ~ ~X                                                                                                                                                             &                                                                         & ~ ~ ~ ~ X~~                                                           & ~ ~ ~ ~ ~X~ ~ ~ ~~                                                           & ~ ~ ~ ~ X                                                         & ~ ~ ~ ~ ~ ~ X                           \\ 
% \hline
% QCovid                                                                                                  & ~ ~ ~ ~ ~ ~ ~  X                &                                                                & ~ ~ ~ ~ X                                                            &                                                                   &                                                                         &                                                                     & ~ ~ ~ ~ ~X                                                                                                                                                        &                                                                         &                                                                       & ~ ~ ~ ~ ~X                                                                   &                                                                   & ~ ~ ~ ~ ~ ~ X                           \\ 
% \hline
% ASIMI Model                                                                                             &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      &                                                                   & ~ ~ ~ ~X                                                                &                                                                     &                                                                                                                                                           &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}19 and Me~\\(Princeton Model)\end{tabular}                                   &  ~ ~ ~ ~ ~ ~ ~  X                & ~ ~ ~ ~X                                                       & ~ ~ ~ ~ X                                                            &                                                                   &                                                                         &                                                                     &                                                                                                                                                           &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         \\ 
% \hline
% MyCOVIDRisk                                                                                             &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      &                                                                   & ~ ~ ~ ~X                                                                &                                                                     &                                                                                                                                                                       & ~ ~ ~ X                                                                 & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Risk\\Assessment Tool~\\(Georgia Tech Model)\end{tabular}           &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      & ~ ~ ~ ~ X                                                         &                                                                         &                                                                     &                                                                                                                                                                          &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         \\ 
% \hline
% Covidtracker.fr                                                                                         &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      &                                                                   &                                                                         &                                                                     &                                                                                                                                                                           &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   & ~ ~ ~ ~ ~ ~ ~X                          \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Morality Risk\\Calculator\\(JHU Model)\end{tabular}                 &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      &                                                                   &                                                                         &                                                                     &                                                                                                                                                            &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              & ~ ~ ~ ~ X                                                         &                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Max Planck Institute - COVID Risk\\Calculator\end{tabular}                   &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      &                                                                   &                                                                         &                                                                     & ~ ~ ~ ~ ~X                                                                                                                                                 &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Indoor Safety\\Guide (MIT Model)\end{tabular}                       &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                &                                                                      &                                                                   &                                                                         &                                                                     & ~ ~ ~ ~ ~X                                                                                                                                                 &                                                                         & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Risk\\Calculator~\\(Northwestern~\\University~\\Model)\end{tabular} &  ~ ~ ~ ~ ~ ~ ~  X                &                                                                & ~ ~ ~ ~X                                                             &                                                                   &                                                                         &                                                                     &                                                                                                                                                            &                                                                         &                                                                       &                                                                              & ~ ~ ~ ~ X                                                         &                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}microCOVID~\\Project\end{tabular}                                            &  ~ ~ ~ ~ ~ ~ ~  X                & ~ ~ ~ ~X                                                       &                                                                      & ~ ~ ~ ~ X                                                         & ~ ~ ~ ~ X                                                               & ~ ~ ~ ~ ~X                                                          &                                                                                                                                                                           & ~ ~ ~ ~X                                                                & ~ ~ ~ ~ X                                                             &                                                                              &                                                                   &                                         
% \hline
% \end{tabular}}
% \end{table}
% \begin{table}
% \centering
% \normalsize
% \begin{tabular}{|l|l|l|} 
% \hline
% \multicolumn{1}{|c|}{\textbf{MODEL}}                                                                                                              & \multicolumn{1}{c|}{\textbf{PROS}}                                                                                                                                                                                                                                                                                                                                                                                                              & \multicolumn{1}{c|}{\textbf{CONS}}                                                                                                                                                                                                                                                                                                                                                                                                                              \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}QCOVID\\ (https://qcovid.org/Calculation)\end{tabular}                                                                 & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Very specific clinical inputs: several options for neurological problems, heart issues, diabetes, etc.\\ Access to algorithm \\ Output includes percentage risk along with risk in terms of odds\\ Outputs both absolute risk and average risk (along with the ratio between the two)\end{tabular}                                                                                                & \begin{tabular}[c]{@{}l@{}}Does not consider vaccination\\ Does not consider mask/mask type\\ Limited location input: only UK postcode\\ Does not consider the amount of people passed \\ Output does not have risk/chance of infection - only risk of death and hospital admission\end{tabular}                                                                                                                                                                \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}ASIMI\\ (https://covid-19.forhealth.org/covid-19-transmission-calculator/)\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}User-friendly UI: Users can use sliders or manually enter values\\ Considers specific environmental factors such as ventilation, air cleaning, and HVAC System\\ Considers behavioral factors such as personal hygiene habits and social distancing\\ The calculator outputs a transmission risk percentage along with a pie chart that visualizes the risks of several different types of transmission\end{tabular} & \begin{tabular}[c]{@{}l@{}}While the calculator considers the type of mask used, the categories are vague and not specific\\ Does not consider vaccination \\ Does not consider a user’s health/medical conditions such as the presence of a chronic illness.\\ Does not consider location (country and/or region)\\ Does not consider the specific number of people passed\\ Does not calculate the risk of death or the risk of hospitalization\end{tabular}  \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Covidtracker\\ (https://covidtracker.fr/covid19-risk-calculator/)\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Uses virus incidence and the number of people to calculate risk of at least one person being COVID positive\\ Provides an explanation for the working of the calculator\end{tabular}                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}Only 2 inputs: does not consider vaccination, mask type, chronic illness, etc.\\ Does not calculate the risk of getting infected with COVID or the risk of hospitalization/death due to COVID\end{tabular}                                                                                                                                                                                                                           \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}19 and Me (Princeton Model)\\ (https://19andme.covid19.mathematica.org/)\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Considers health/medical conditions such as underlying health issues\\ Considers vaccination\\ Considers behavioral factors\end{tabular}                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Does not calculate risk of hospitalization or risk of death\\ Very limited options for location - only US and Belgium pincode option\\ Does not consider environmental factors (ventilation, indoor/outdoor, etc)\\ Does not consider mask/mask type\end{tabular}                                                                                                                                                                    \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}MyCOVIDRisk\\ (https://mycovidrisk.app/)\end{tabular}                                                                  & \begin{tabular}[c]{@{}l@{}}User-friendly and interactive UI\\ Considers specific activities (going to the gym, going grocery shopping, etc)\\ Considers if others are wearing a mask\end{tabular}                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}Does not consider medical/health conditions of user\\ Does not consider vaccination\\ Does not consider mask types\\ Limited to within the United States\\ Does not consider the number of people passed\\ Does not calculate risk of hospitalization or risk of death\end{tabular}                                                                                                                                                  \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Event RIsk Assessment Planning Tool (Georgia Tech)\\ (https://covid19risk.biosci.gatech.edu/)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}User-friendly and interactive UI\\ Uses location and size of the gathering to calculate the risk of coming into contact with a person who has COVID-19\end{tabular}                                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}Does not consider health/medical conditions of user\\ Does not consider vaccination\\ Does not consider masks/mask types\\ Does not consider environmental factors\\ Does not calculate risk of hospitalization or risk of death\end{tabular}                                                                                                                                                                                        \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Mortality Risk Calculator - JHU Model\\ https://covid19risktools.com:8443/riskcalculator\end{tabular}         & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Considers information about user - age, ethnicity, smoking habit, height, weight, etc\\ Considers medical/health conditions of user\\ Calculates individualized risks for mortality from COVID\end{tabular}                                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Does not consider mask/mask type\\ Does not consider vaccination\\ Does not calculate risk of hospitalization\\ Does not consider number of people passed\end{tabular}                                                                                                                                                                                                                                                               \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Max Planck Institute - COVID Risk Calculator\\ https://www.mpic.de/4747361/risk-calculator?en\end{tabular}             & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Considers properties of the infectious person\\ Considers environmental factors/properties\\ Considers aerosol and virus properties\end{tabular}                                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}Does not calculate risk of death or risk of hospitalization\\ Does not consider mask types\\ Does not consider location\\ Does not consider vaccination details\end{tabular}                                                                                                                                                                                                                                                         \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Indoor Safety Guideline - MIT Model\\ https://indoor-covid-safety.herokuapp.com\\ /\end{tabular}              & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Calculates the limits of safe occupancy following the entrance of a single infected person into an indoor space\\ Considers environmental factors (properties of the room)\\ Considers behavioral factors\end{tabular}                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Does not consider vaccination\\ Does not consider location\\ Limited to indoors \\ Does not consider health/medical conditions of the user\end{tabular}                                                                                                                                                                                                                                                                              \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}COVID-19 Risk Calculator - Northwestern University\\ https://fightcovidmilwaukee.org/risk-assessment-tool\end{tabular} & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Visualization present\\ Considers information about user (age, height, gender, etc)\\ Considers medical/health condition of user\\ Calculates life expectancy loss for COVID and risk of death from COVID\end{tabular}                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Does not consider vaccination\\ Does not consider location\\ Does not consider environmental factors\\ Does not consider mask/mask type\\ Does not calculate risk of infection or risk of hospitalization\end{tabular}                                                                                                                                                                                                               \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}microCOVID Project\\ (https://www.microcovid.org/)\end{tabular}                                                        & \begin{tabular}[c]{@{}l@{}}User-friendly UI\\ Considers location\\ Considers specific activities (such as grocery shopping, going to a bar, etc)\\ Considers number of people within 15 feet\\ Considers vaccination status of user and of people around the user\\ Considers mask type(s) of user and of people around user\end{tabular}                                                                                                       & \begin{tabular}[c]{@{}l@{}}Does not consider medical/health conditions of user\\ Does not calculate risk of hospitalization or risk of death\end{tabular}                                                                                                                                                                                                                                                                                                      \\
% \hline
% \end{tabular}
% \end{table}


==> ratio_survey_diff.tex <==
\begin{longtable}{|l|l|l|l|l|l|l|l|} 
\hspace*{-5cm}
\scalebox{0.1}{
\hline
 & \textbf{ISO\_3} & \textbf{Ox\_active\_calc\_perpop} & \textbf{max\_ox\_active\_calc\_perpop} & \textbf{max\_pcli} & \textbf{ISO2} & \textbf{Survey\_Reported\_Ratio} & \textbf{Country}        \\ 
\hline
1   & BRA             & 0.000211050904147                 & 0.002968995723205                      & 0.048076785623473  & BR            & 16.1929453948727                 & Brazil                  \\ 
\hline
2   & ARG             & 4.03387904617555E-05              & 0.004380083981177                      & 0.041989750779322  & AR            & 9.58651728135145                 & Argentina               \\ 
\hline
3   & AUS             & 1.32269509259616E-05              & 0.000258359718701                      & 0.024025305835929  & AU            & 1                                & Australia               \\ 
\hline
4   & AUT             & 0.000126322896869                 & 0.01061058403783                       & 0.010129640575311  & AT            & 0.954673233744341                & Austria                 \\ 
\hline
5   & BEL             & 0.001318876870653                 & 0.018468923203357                      & 0.01670914850298   & BE            & 0.904716984255076                & Belgium                 \\ 
\hline
6   & BGD             & 3.31689349311086E-05              & 0.000308776084595                      & 0.132592712286006  & BD            & 429.413801460121                 & Bangladesh              \\ 
\hline
7   & BGR             & 9.6424451801806E-05               & 0.006644693267959                      & 0.030949950548888  & BG            & 4.65784488474865                 & Bulgaria                \\ 
\hline
8   & BHR             & 0.000816386499063                 & 0.005697998283103                      & 0.003922170288214  & BH            & 0.688341781331313                & Bahrain                 \\ 
\hline
9   & BHS             & 8.00160328421361E-05              & 0.003552563680352                      & 0.004410231361019  & BS            & 1.24142218348115                 & Bahamas                 \\ 
\hline
10  & BLR             & 0.000940800621937                 & 0.002769303418829                      & 0.099379456348889  & BY            & 35.8860844475101                 & Belarus                 \\ 
\hline
11  & BOL             & 5.90739474015706E-05              & 0.001824230909401                      & 0.089055668437124  & BO            & 48.8181994824169                 & Bolivia                 \\ 
\hline
13  & CAN             & 0.000630870950594                 & 0.002450265178672                      & 0.008333888218824  & CA            & 3.40121889310754                 & Canada                  \\ 
\hline
14  & CHL             & 0.000411386282094                 & 0.00445001000535                       & 0.019884002764518  & CL            & 4.46830518147418                 & Chile                   \\ 
\hline
15  & COL             & 5.80997985017344E-05              & 0.003047631191284                      & 0.068900171726872  & CO            & 22.6077787640216                 & Colombia                \\ 
\hline
16  & CRI             & 1.76113481694546E-05              & 0.003303249523694                      & 0.049349277190471  & CR            & 14.9396153201527                 & Costa Rica              \\ 
\hline
17  & CZE             & 0.000126902830437                 & 0.015685926206638                      & 0.022649714307652  & CZ            & 1.44395134908054                 & Czech Republic          \\ 
\hline
18  & DEU             & 0.000329993339978                 & 0.003711440825464                      & 0.007384824850435  & DE            & 1.98974608453074                 & Germany                 \\ 
\hline
19  & DNK             & 0.000404830001243                 & 0.006654908000199                      & 0.012918390539979  & DK            & 1.9411824385239                  & Denmark                 \\ 
\hline
20  & ECU             & 0.00092705848189                  & 0.00113180923374                       & 0.06087249014929   & EC            & 53.7833482309971                 & Ecuador                 \\ 
\hline
21  & EGY             & 2.62598462417948E-05              & 0.000208155104626                      & 0.095173607025697  & EG            & 457.224468248504                 & Egypt                   \\ 
\hline
22  & ESP             & 0.000762079485071                 & 0.005992328741247                      & 0.010656762911071  & ES            & 1.77840091410844                 & Spain                   \\ 
\hline
23  & FIN             & 0.000289776676781                 & 0.001117183326355                      & 0.013928870881573  & FI            & 12.4678470873903                 & Finland                 \\ 
\hline
24  & FRA             & 0.000721382106398                 & 0.009784279655407                      & 0.01491971570518   & FR            & 1.52486603313054                 & France                  \\ 
\hline
25  & GBR             & 0.000964436020342                 & 0.00490288050656                       & 0.015385348664229  & GB            & 3.13802236127194                 & United Kingdom          \\ 
\hline
26  & GHA             & 3.5745387649649E-05               & 0.000303061120061                      & 0.050865048765871  & GH            & 167.837592481574                 & Ghana                   \\ 
\hline
27  & GRC             & 3.79515858376469E-05              & 0.003368700081295                      & 0.010311792218691  & GR            & 3.06105974703642                 & Greece                  \\ 
\hline
28  & GTM             & 2.09554378308615E-05              & 0.000878214650281                      & 0.039534169239048  & GT            & 45.0165221297275                 & Guatemala               \\ 
\hline
29  & HND             & 2.96254633251548E-05              & 0.001125983955893                      & 0.047203036443796  & HN            & 41.921588843908                  & Honduras                \\ 
\hline
30  & HUN             & 0.000116174424127                 & 0.007678543830491                      & 0.017168462752389  & HU            & 2.23590085977158                 & Hungary                 \\ 
\hline
31  & IDN             & 1.69648449340863E-05              & 0.000316529995304                      & 0.069210989689268  & ID            & 218.655390377271                 & Indonesia               \\ 
\hline
32  & IND             & 1.45377384848983E-05              & 0.000927255645744                      & 0.066435053336072  & IN            & 71.6469655817082                 & India                   \\ 
\hline
33  & IRL             & 0.001693616184605                 & 0.002935294713634                      & 0.013693784544534  & IE            & 4.66521623226707                 & Ireland                 \\ 
\hline
34  & ISR             & 0.000395271432013                 & 0.009146913341744                      & 0.012164055913155  & IL            & 1.32985363025601                 & Israel                  \\ 
\hline
35  & ITA             & 0.000645647056706                 & 0.00792247468203                       & 0.008041603327587  & IT            & 1.01503679725572                 & Italy                   \\ 
\hline
36  & JOR             & 5.37649930473743E-06              & 0.007171676019209                      & 0.080282499982571  & JO            & 11.1943846553502                 & Jordan                  \\ 
\hline
37  & JPN             & 4.32378593244432E-05              & 0.000275737362024                      & 0.005269611496425  & JP            & 19.1109810355109                 & Japan                   \\ 
\hline
38  & MEX             & 8.89167837305523E-05              & 0.001119701080587                      & 0.026588702419603  & MX            & 23.7462505668625                 & Mexico                  \\ 
\hline
39  & NIC             & 6.46943822288155E-07              & 0.000127728275314                      & 0.080270458998641  & NI            & 628.447059208                    & Nicaragua               \\ 
\hline
40  & NLD             & 0.000648793874854                 & 0.007620891477917                      & 0.010923701895124  & NL            & 1.43338898431728                 & Netherlands             \\ 
\hline
41  & NOR             & 0.000178741361987                 & 0.001495203246426                      & 0.013841787763127  & NO            & 9.25746235250211                 & Norway                  \\ 
\hline
42  & NPL             & 1.35760412221085E-06              & 0.001774897053693                      & 0.117940746716866  & NP            & 66.4493450318547                 & Nepal                   \\ 
\hline
43  & NZL             & 2.2870258298534E-05               & 0.00019907789607                       & 0.025490675597324  & NZ            & 1                                & New Zealand             \\ 
\hline
44  & PAK             & 4.32570131546565E-05              & 0.000346246243112                      & 0.105865828417517  & PK            & 305.753002447385                 & Pakistan                \\ 
\hline
45  & PAN             & 0.000614765856087                 & 0.007355901257241                      & 0.041608440150198  & PA            & 5.65647072943543                 & Panama                  \\ 
\hline
46  & PER             & 0.000659410902402                 & 0.003412005368492                      & 0.085365566576177  & PE            & 25.0191770987452                 & Peru                    \\ 
\hline
47  & PHL             & 2.58882025495053E-05              & 0.000537210839057                      & 0.026735592097618  & PH            & 49.7674100257406                 & Philippines             \\ 
\hline
48  & POL             & 0.00013055330106                  & 0.00878268485236                       & 0.032817668743274  & PL            & 3.73663285145154                 & Poland                  \\ 
\hline
49  & PRT             & 0.000666853813884                 & 0.008035505797578                      & 0.006201750637273  & PT            & 0.771793436965994                & Portugal                \\ 
\hline
50  & PSE             & 1.32496075353218E-05              & 0.005780565149137                      & 0.101575398987982  & PS            & 17.5718803209326                 & Palestine               \\ 
\hline
51  & ROU             & 0.000242225386761                 & 0.006034574820559                      & 0.017647077348347  & RO            & 2.92432820423844                 & Romania                 \\ 
\hline
52  & RUS             & 0.000492735861507                 & 0.002615697644957                      & 0.048762387010465  & RU            & 18.6422108474512                 & Russia                  \\ 
\hline
53  & SDN             & 6.68849860375555E-06              & 8.61262294636541E-05                   & 0.092291919950901  & SD            & 1071.58899821393                 & Sudan                   \\ 
\hline
54  & SLV             & 3.09888447867436E-05              & 0.000892619688356                      & 0.065421509235043  & SV            & 73.2915821692448                 & El Salvador             \\ 
\hline
55  & SRB             & 0.000456577351962                 & 0.011444289134569                      & 0.030010289004886  & RS            & 2.62229384909855                 & Serbia                  \\ 
\hline
56  & SWE             & 0.00081976262629                  & 0.008333194827261                      & 0.024915487516263  & SE            & 2.9899081964043                  & Sweden                  \\ 
\hline
57  & THA             & 4.67253524267382E-06              & 2.254810370939E-05                     & 0.018073049728426  & TH            & 801.533022969904                 & Thailand                \\ 
\hline
58  & TUR             & 0.000588759519612                 & 0.014604472342913                      & 0.021096028594339  & TR            & 1.44449098187216                 & Turkey                  \\ 
\hline
59  & TWN             & 1.55352687339071E-06              & 9.7770224078257E-06                    & 0.003983534393631  & TW            & 407.438402763826                 & Taiwan                  \\ 
\hline
60  & UKR             & 0.000137014118683                 & 0.004400176817953                      & 0.065424920699936  & UA            & 14.8687026469015                 & Ukraine                 \\ 
\hline
61  & URY             & 3.73826241121627E-05              & 0.001429957341039                      & 0.026299109216286  & UY            & 18.3915341119101                 & Uruguay                 \\ 
\hline
62  & VNM             & 5.2834725919485E-08               & 4.18568439784365E-06                   & 0.013842923709934  & VN            & 3307.20675382634                 & Vietnam                 \\ 
\hline
63  & ZAF             & 4.54329952081462E-05              & 0.00285277876528                       & 0.072690380590961  & ZA            & 25.4805530227746                 & South Africa            \\ 
\hline
64  & ARE             & 0.000667949160639                 & 0.001906971454316                      & 0.034843923534452  & AE            & 18.2718642460967                 & United Arab Emirates    \\ 
\hline
77  & CHE             & 0.00035348576914                  & 0.012451942689451                      & 0.012413817037011  & CH            & 0.996938176364119                & Switzerland             \\ 
\hline
84  & DOM             & 0.000290826264493                 & 0.001794526055513                      & 0.073281540597163  & DO            & 40.8361530176973                 & Dominican Republic      \\ 
\hline
95  & HRV             & 7.98625626194698E-05              & 0.011852648247796                      & 0.036416428871205  & HR            & 3.07242973130297                 & Croatia                 \\ 
\hline
100 & IRQ             & 1.44943775613312E-05              & 0.001494192387755                      & 0.148951062800909  & IQ            & 99.6866695490737                 & Iraq                    \\ 
\hline
105 & KAZ             & 0.000102261959839                 & 0.001969834220665                      & 0.085098310365332  & KZ            & 43.2007472875579                 & Kazakhstan              \\ 
\hline
106 & KOR             & 3.50530802692272E-06              & 0.000217696904235                      & 0.01139136020158   & KR            & 52.3266981752393                 & South Korea             \\ 
\hline
107 & LBY             & 3.11856737006785E-06              & 0.001907710822067                      & 0.067891908484291  & LY            & 35.5881550279871                 & Libya                   \\ 
\hline
108 & LKA             & 1.87000380665527E-05              & 0.00044077517482                       & 0.027753478548509  & LK            & 62.9651580533637                 & Sri Lanka               \\ 
\hline
109 & MAR             & 6.04201848236076E-05              & 0.001916280869215                      & 0.046463780811088  & MA            & 24.2468531401294                 & Morocco                 \\ 
\hline
110 & MDA             & 0.000653246598806                 & 0.007506113974813                      & 0.046668378726536  & MD            & 6.2173821078563                  & Moldova                 \\ 
\hline
112 & MYS             & 2.80188213210148E-05              & 0.000619406627483                      & 0.01750950565672   & MY            & 28.2681922985958                 & Malaysia                \\ 
\hline
113 & NGA             & 6.53995122277486E-06              & 4.13686392171583E-05                   & 0.067567174384975  & NG            & 1633.29458410008                 & Nigeria                 \\ 
\hline
125 & PRY             & 1.45610360375427E-05              & 0.001653608935757                      & 0.072628911942766  & PY            & 43.9214558970095                 & Paraguay                \\ 
\hline
127 & QAT             & 0.003038075711504                 & 0.008657053018958                      & 0.030459293915506  & QA            & 3.51843679931294                 & Qatar                   \\ 
\hline
130 & SAU             & 0.000441933865138                 & 0.001586350452094                      & 0.043005975585144  & SA            & 27.1100093477891                 & Saudi Arabia            \\ 
\hline
134 & SVK             & 8.94093160582429E-05              & 0.005954315057916                      & 0.019250820944166  & SK            & 3.233087392407                   & Slovak Republic         \\ 
\hline
141 & UZB             & 2.29763463444289E-05              & 0.000298351037178                      & 0.074873849026962  & UZ            & 250.958903093366                 & Uzbekistan              \\ 
\hline
142 & VEN             & 4.70229877100197E-06              & 0.000520422897422                      & 0.05567123141264   & VE            & 106.973063038601                 & Venezuela               \\ 
\hline
145 & AFG             & 3.3842397810289E-05               & 0.000250093191365                      & 0.22389290424889   & AF            & 895.237903225526                 & Afghanistan             \\ 
\hline
146 & AGO             & 2.8253019647967E-07               & 0.000104631798302                      & 0.035133087215225  & AO            & 335.778298616946                 & Angola                  \\ 
\hline
147 & ALB             & 8.87583701798881E-05              & 0.003792335397032                      & 0.044447646583989  & AL            & 11.7203891350905                 & Albania                 \\ 
\hline
153 & BFA             & 4.85911601362277E-06              & 7.63175084727504E-05                   & 0.045966692025609  & BF            & 602.308604479953                 & Burkina Faso            \\ 
\hline
158 & BIH             & 0.000169687594992                 & 0.006603316340915                      & 0.037777742000953  & BA            & 5.72102562569583                 & Bosnia and Herzegovina  \\ 
\hline
165 & CIV             & 2.19932076353008E-05              & 0.000150480981865                      & 0.048643816010521  & CI            & 323.255572947449                 & Cote d'Ivoire           \\ 
\hline
172 & DZA             & 3.87057082218091E-05              & 0.000329130460057                      & 0.081164668773726  & DZ            & 246.603334008002                 & Algeria                 \\ 
\hline
182 & HKG             & 2.66774052115111E-06              & 0.000221441518545                      & 0.008399269445336  & HK            & 37.9299667945044                 & Hong Kong               \\ 
\hline
194 & KEN             & 3.10043272370236E-06              & 0.000270547957143                      & 0.080126855432476  & KE            & 296.165072834831                 & Kenya                   \\ 
\hline
195 & KGZ             & 4.26354835791188E-05              & 0.003514905455532                      & 0.104143446007853  & KG            & 29.6290888404785                 & Kyrgyz Republic         \\ 
\hline
196 & KHM             & 0                                 & 6.13907253078724E-06                   & 0.065003749009711  & KH            & 10588.5292417901                 & Cambodia                \\ 
\hline
198 & KWT             & 0.00058750925813                  & 0.002915836246321                      & 0.043739409870228  & KW            & 15.0006400137941                 & Kuwait                  \\ 
\hline
199 & LBN             & 9.73248944626635E-06              & 0.003371941316647                      & 0.047512349208846  & LB            & 14.0905029913437                 & Lebanon                 \\ 
\hline
205 & MOZ             & 1.48545593521803E-06              & 8.80121215032567E-05                   & 0.045744240022693  & MZ            & 519.749316814273                 & Mozambique              \\ 
\hline
213 & OMN             & 0.000260613787432                 & 0.004055263550868                      & 0.022735725594997  & OM            & 5.60647299732993                 & Oman                    \\ 
\hline
219 & PRI             & -3.51543503183941E-05             & 0.003802012896154                      & 0.021194495893537  & PR            & 5.57454602928327                 & Puerto Rico             \\ 
\hline
228 & SEN             & 3.96196581300165E-05              & 0.000116624342774                      & 0.046984896498433  & SN            & 402.873837321647                 & Senegal                 \\ 
\hline
229 & SGP             & 0.002005059826295                 & 0.002005059826295                      & 0.012263851950391  & SG            & 6.11645188316077                 & Singapore               \\ 
\hline
233 & SVN             & 7.35265519496699E-05              & 0.011074610484502                      & 0.021594383836941  & SI            & 1.94990007704214                 & Slovenia                \\ 
\hline
236 & TUN             & 1.51576810406408E-05              & 0.001747110095641                      & 0.054396758771814  & TN            & 31.1352781416284                 & Tunisia                 \\ 
\hline
253 & BEN             & 3.57962914871561E-06              & 5.83698712208933E-05                   & 0.041594827435358  & BJ            & 712.607832865476                 & Benin                   \\ 
\hline
263 & BWA             & 3.03741075555653E-06              & 0.001162963830087                      & 0                  & BW            & 1                                & Botswana                \\ 
\hline
268 & CMR             & 3.53781249132061E-05              & 0.000148890566166                      & 0.067462783719558  & CM            & 453.103144523297                 & Cameroon                \\ 
\hline
308 & MLI             & 1.60205050048347E-05              & 5.61035122428227E-05                   & 0.046188270348503  & ML            & 823.268784823928                 & Mali                    \\ 
\hline
343 & TZA             & 5.32358187061225E-06              & 5.38097897972936E-06                   & 0.096572707793277  & TZ            & 17947.0516716521                 & Tanzania                \\ 
\hline
384 & ETH             & 3.08669870403569E-07              & 0.000189433053728                      & 0.09338620974582   & ET            & 492.977375953172                 & Ethiopia                \\ 
\hline
408 & LAO             & 0                                 & 2.06169696903056E-06                   & 0.023158181656475  & LA            & 11232.5826755053                 & Laos                    \\ 
\hline
456 & YEM             & 3.25829593097838E-07              & 1.63516328105408E-05                   & 0.097620410463999  & YE            & 5970.07109902015                 & Yemen                   \\ 
\hline
497 & GIN             & 8.62830333666893E-05              & 9.53739371223154E-05                   & 0.018597789607066  & GN            & 194.998656532498                 & Guinea                  \\ 
\hline
574 & AZE             & 5.58853714017374E-05              & 0.005691294568407                      & 0.044953830402012  & AZ            & 7.89870035045325                 & Azerbaijan              \\ 
\hline
634 & MDG             & 1.16076834527561E-06              & 0.000165375955894                      & 0.068422690312652  & MG            & 413.740255908173                 & Madagascar              \\ 
\hline
638 & MRT             & 2.1506958146169E-07               & 0.000599337475082                      & 0.012355573020168  & MR            & 20.6153853777947                 & Mauritania              \\ 
\hline
639 & USA             & N/A                               & N/A                                    & N/A                & US            & 3                                & United States           \\
\hline
\caption{Ratio of Reported Cases from Facebook Surveys to Reported Number of Cases}
}
\end{longtable}


==> vaccine_table.tex <==
\begin{table}[]
\scalebox{0.7}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Vaccine} & \textbf{Normal} & \textbf{Alpha} & \textbf{Beta} & \textbf{Gamma} & \textbf{Delta} & \textbf{Omicron} \\ 
\hline
Pfizer (Dose 1) & 0.8 - 0.91 & 0.49 & 0.36-0.375 & 0.36-0.37 & 0.33 & - \\ 
\hline
Pfizer (Dose 2) & 0.95 & 0.87-0.95 & 0.72-0.85 & 0.75-0.77 & 0.79 - 0.92 & 0.07-0.1 \\
\hline
Pfizer (Dose 2) + Pfizer Booster & 0.95 & 0.87-0.95 & 0.72-0.85 & 0.75-0.77 & 0.79-0.92 & 0.44-0.47 \\ \hline
Pfizer (Dose 2) + Moderna (Booster) & 0.95 & 0.87-0.95 & 0.72-0.85 & 0.75-0.77 & 0.79-0.92 & 0.63-0.66 \\ \hline
Moderna (Dose 1) & 0.8-0.9 & 0.49 & 0.72 & 0.72 & 0.33 & - \\ \hline
Moderna (Dose 2) & 0.9-0.96 & 0.91-0.96 & 0.9-0.96 & 0.9-0.96 & 0.855-0.96 & 0.35-0.52 \\ \hline
J\&J (Dose 1) & 0.69-0.77 & 0.77 & 0.52-0.57 & 0.51-0.68 & 0.49-0.78 & - \\ \hline
J\&J (Dose 1) + J\&J Booster & 0.69-0.77 & 0.77 & 0.52-0.57 & 0.51-0.68 & 0.49-0.78 & 0.85 \\ \hline
Astrazeneca (Dose 1) & 0.55-0.67 & 0.33-0.37 & 0.1-0.11 & 0.11-0.243 & 0.329 & - \\ \hline
Astrazeneca (Dose 2) & 0.82-0.85 & 0.66-0.74 & 0.22-0.49 & 0.22-0.49 & 0.59 & - \\ \hline
Astrazeneca (Dose 2) + Pfizer/Moderna (Booster) & 0.82-0.85 & 0.66-0.74 & 0.22-0.7 & 0.22-0.49 & 0.59 & 0.59-0.62\\ \hline
Novavax (Dose 1) & 0.904 & 0.863 & 0.486 & - & - & - \\ \hline
No Vaccine & 0 & 0 & 0 & 0 & 0 & 0\\ \hline
\end{tabular}}
\caption{\label{tab:vaccine_eff}Vaccine Efficacy based on Dosage and Manufacturing Company, - represents that the efficacy is currently under investigation and a valid source for the same has not yet been found by us.}
\end{table}


==> vaccine_table_old.tex <==
\begin{table}[]
\scalebox{0.75}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Vaccine}                                & \textbf{Normal} & \textbf{Alpha} & \textbf{Beta} & \textbf{Gamma} & \textbf{Delta} & \textbf{Omicron} & \textbf{normal\_u} & \textbf{alpha\_u} & \textbf{beta\_u} & \textbf{gamma\_u} & \textbf{delta\_u} & \textbf{omicron\_u} \\ \hline
Pfizer (Dose 1)                                 & 0.8             & 0.49           & 0.36          & 0.36           & 0.33           & 0.44             & 0.91               & 0.49              & 0.375            & 0.37              & 0.33              & 0.44                \\ \hline
Pfizer (Dose 2)                 & 0.95            & 0.87           & 0.72          & 0.75           & 0.79           & 0.88             & 0.95               & 0.95              & 0.85             & 0.77              & 0.92              & 0.88                \\ \hline
Pfizer (Dose 2) + Pfizer Booster                & 0.95            & 0.87           & 0.72          & 0.75           & 0.79           & 0.49             & 0.95               & 0.95              & 0.85             & 0.77              & 0.92              & 0.65                \\ \hline
Pfizer (Dose 2) + Moderna (Booster)             & 0.95            & 0.87           & 0.72          & 0.75           & 0.79           & 0.57             & 0.95               & 0.95              & 0.85             & 0.77              & 0.92              & 0.7                 \\ \hline
Moderna (Dose 1)                                & 0.8             & 0.49           & 0.72          & 0.72           & 0.33           &                  & 0.9                & 0.49              & 0.49             & 0.49              & 0.49              &                     \\ \hline
Moderna (Dose 2)                                & 0.9             & 0.91           & 0.9           & 0.9            & 0.855          &                  & 0.96               & 0.96              & 0.96             & 0.96              & 0.96              &                     \\ \hline
J\&J (Dose 1)                                   & 0.69            & 0.77           & 0.52          & 0.51           & 0.49           &                  & 0.77               & 0.77              & 0.57             & 0.68              & 0.78              &                     \\ \hline
J\&J (Dose 1) + J\&J Booster                    & 0.69            & 0.77           & 0.52          & 0.51           & 0.49           & 0.85             & 0.77               & 0.77              & 0.57             & 0.68              & 0.78              & 0.85                \\ \hline
Astrazeneca (Dose 1)                            & 0.55            & 0.33           & 0.1           & 0.11           & 0.329          &                  & 0.67               & 0.37              & 0.11             & 0.243             & 0.329             &                     \\ \hline
Astrazeneca (Dose 2)                            & 0.82            & 0.66           & 0.22          & 0.22           & 0.598          &                  & 0.85               & 0.74              & 0.7              & 0.486             & 0.598             &                     \\ \hline
Astrazeneca (Dose 2) + Pfizer/Moderna (Booster) & 0.82            & 0.66           & 0.22          & 0.22           & 0.598          & 0.56             & 0.85               & 0.74              & 0.7              & 0.486             & 0.598             & 0.65                \\ \hline
Novavax (Dose 1)                                & 0.904           & 0.863          & 0.486         &                &                &                  & 0.91               & 0.863             & 0.486            &                   &                   &                     \\ \hline
No Vaccine                                      & 0               & 0              & 0             & 0              & 0              & 0                & 0                  & 0                 & 0                & 0                 & 0                 & 0                   \\ \hline
\end{tabular}}
\caption{\label{tab:mask_ffe}Vaccine Efficacy based on Dosage and Manufacturing Company}
\end{table}

\begin{table}
\centering
\scalebox{0.90}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|} 
\hline
Dose 1      & Dose 2      & Booster Dose   & Normal      & Alpha       & Beta        & Gamma       & Delta       & Omicron      \\ 
\hline
Pfizer~     & Pfizer      &                & 0.950       & 0.870-0.950 & 0.720-0.850 & 0.750-0.770 & 0.790-0.920 & 0.880        \\ 
\hline
Moderna     & Moderna     &                & 0.900-0.960 & 0.910-0.960 & 0.900-0.960 & 0.900-0.960 & 0.855-0.960 & -            \\ 
\hline
JJ          &             &                & 0.690-0.770 & 0.770       & 0.520-0.570 & 0.510-0.680 & 0.490-0.780 & -            \\ 
\hline
Astrazeneca & Astrazeneca &                & 0.820-0.850 & 0.660-0.740 & 0.220-0.700 & 0.220-0.486 & 0.598       & -            \\ 
\hline
Novavax     &             &                & 0.904-0.910 & 0.000-0.863 & 0.000-0.486 & -           & -           & -            \\ 
\hline
Astrazeneca & Astrazeneca & Pfizer/Moderna & -           & -           & -           & -           & -           & 0.480-0.560  \\ 
\hline
Pfizer      & Pfizer      & Pfizer         & -           & -           & -           & -           & -           & 0.490        \\ 
\hline
Pfizer      & Pfizer      & Moderna        & -           & -           & -           & -           & -           & 0.570        \\ 
\hline
JJ          & JJ          & JJ             & -           & -           & -           & -           & -           & 0.850        \\ 
\hline
            &             &                &             &             &             &             &             &              \\ 
\hline
            &             &                &             &             &             &             &             &              \\
\hline
\end{tabular}}
\end{table}

